Bayesian Model Averaging in Causal Instrumental Variable Models

Instrumental variables are a popular tool to infer causal effects under unobserved confounding, but choosing suitable instruments is challenging in practice. We propose gIVBMA, a Bayesian model averaging procedure that addresses this challenge by averaging across different sets of instrumental variables and covariates in a structural equation model. This allows for data-driven selection of valid and relevant instruments and provides additional robustness against invalid instruments. Our approach extends previous work through a scale-invariant prior structure and accommodates non-Gaussian outcomes and treatments, offering greater flexibility than existing methods. The computational strategy uses conditional Bayes factors to update models separately for the outcome and treatments. We prove that this model selection procedure is consistent. In simulation experiments, gIVBMA outperforms current state-of-the-art methods. We demonstrate its usefulness in two empirical applications: the effects of malaria and institutions on income per capita and the returns to schooling. A software implementation of gIVBMA is available in Julia.

==> table_1.tex <==
\begin{table}[h]
\centering
\begin{tabular}{l*{8}{r}}
\toprule
 & \multicolumn{8}{c}{$n = 50$} \\
 & \multicolumn{4}{c}{$s = 3$} & \multicolumn{4}{c}{$s = 6$} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}
 & \textbf{MAE} & \textbf{Bias} & \textbf{Cov.} & \textbf{LPS} & \textbf{MAE} & \textbf{Bias} & \textbf{Cov.} & \textbf{LPS} \\
\midrule
BMA (hyper-g/n) & 0.47 & 0.47 & 0.1 & 1.39 & 0.47 & 0.47 & 0.08 & \textbf{1.41} \\
gIVBMA (BRIC, IW) & 0.3 & 0.29 & \textbf{0.93} & 1.39 & 0.24 & 0.22 & 0.99 & \textbf{1.41} \\
gIVBMA (hyper-$g/n$, IW) & 0.14 & 0.06 & 0.9 & 1.4 & 0.17 & \textbf{0.01} & 0.99 & \textbf{1.41} \\
gIVBMA (BRIC, $\omega_a = 0.1$) & 0.42 & 0.42 & 0.85 & 1.38 & 0.42 & 0.42 & \textbf{0.95} & \textbf{1.41} \\
gIVBMA (hyper-$g/n$, $\omega_a = 0.1$) & 0.33 & 0.33 & 0.92 & 1.39 & 0.33 & 0.33 & 0.99 & \textbf{1.41} \\
gIVBMA (BRIC, $\omega_a = 1$) & 0.24 & 0.23 & 0.9 & 1.39 & 0.26 & 0.2 & 0.97 & \textbf{1.41} \\
gIVBMA (hyper-$g/n$, $\omega_a = 1$) & 0.18 & \textbf{0.01} & 0.91 & 1.4 & 0.24 & 0.09 & \textbf{0.95} & \textbf{1.41} \\
gIVBMA (BRIC, $\omega_a = 10$) & 0.47 & 0.02 & 0.83 & 1.39 & 0.59 & 0.03 & 0.92 & \textbf{1.41} \\
gIVBMA (hyper-$g/n$, $\omega_a = 10$) & 0.33 & 0.21 & 0.86 & 1.4 & 0.62 & 0.28 & 0.81 & \textbf{1.41} \\
BayesHS & 0.37 & 0.37 & 0.38 & 1.78 & 0.49 & 0.49 & 0.37 & 1.83 \\
TSLS & 1.25 & 1.25 & 0.18 & 2.17 & 2.43 & 2.43 & 0.09 & 2.41 \\
O-TSLS & 0.21 & 0.2 & 0.79 & 1.43 & 0.3 & 0.27 & 0.89 & 1.54 \\
IVBMA & \textbf{0.08} & 0.04 & 0.99 & \textbf{1.37} & \textbf{0.13} & 0.12 & 1.0 & 1.46 \\
sisVIVE & 0.6 & 0.6 & - & 1.64 & 2.2 & 2.2 & - & 2.37 \\
\midrule
 & \multicolumn{8}{c}{$n = 500$} \\
 & \multicolumn{4}{c}{$s = 3$} & \multicolumn{4}{c}{$s = 6$} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}
 & \textbf{MAE} & \textbf{Bias} & \textbf{Cov.} & \textbf{LPS} & \textbf{MAE} & \textbf{Bias} & \textbf{Cov.} & \textbf{LPS} \\
\midrule
BMA (hyper-g/n) & 0.46 & 0.46 & 0.0 & 1.3 & 0.48 & 0.48 & 0.0 & \textbf{1.28} \\
gIVBMA (BRIC, IW) & 0.1 & 0.06 & 0.98 & 1.29 & 0.21 & 0.2 & 0.97 & \textbf{1.28} \\
gIVBMA (hyper-$g/n$, IW) & 0.08 & 0.06 & 0.94 & 1.29 & 0.21 & 0.18 & \textbf{0.94} & \textbf{1.28} \\
gIVBMA (BRIC, $\omega_a = 0.1$) & 0.1 & 0.09 & 0.93 & 1.29 & 0.16 & 0.16 & 0.89 & \textbf{1.28} \\
gIVBMA (hyper-$g/n$, $\omega_a = 0.1$) & 0.09 & 0.08 & 0.92 & 1.29 & 0.17 & 0.17 & 0.89 & \textbf{1.28} \\
gIVBMA (BRIC, $\omega_a = 1$) & 0.08 & 0.06 & 0.93 & 1.29 & 0.2 & 0.18 & 0.96 & \textbf{1.28} \\
gIVBMA (hyper-$g/n$, $\omega_a = 1$) & 0.1 & 0.07 & \textbf{0.95} & 1.29 & 0.19 & 0.18 & 0.93 & \textbf{1.28} \\
gIVBMA (BRIC, $\omega_a = 10$) & 0.1 & 0.07 & 0.97 & 1.29 & 0.32 & 0.31 & 0.89 & \textbf{1.28} \\
gIVBMA (hyper-$g/n$, $\omega_a = 10$) & 0.11 & 0.08 & 0.93 & 1.29 & 0.52 & 0.52 & 0.7 & \textbf{1.28} \\
BayesHS & 0.35 & 0.35 & 0.04 & 1.34 & 0.51 & 0.51 & 0.02 & 1.3 \\
TSLS & 1.82 & 1.82 & 0.0 & 2.2 & 3.63 & 3.63 & 0.0 & 2.7 \\
O-TSLS & \textbf{0.07} & \textbf{0.04} & 0.92 & 1.42 & \textbf{0.08} & \textbf{0.05} & 0.96 & 1.4 \\
IVBMA & 0.09 & 0.08 & 0.78 & \textbf{1.28} & 0.09 & 0.06 & 0.74 & 1.3 \\
sisVIVE & 0.21 & 0.21 & - & 1.61 & 4.36 & 4.36 & - & 3.07 \\
\bottomrule
\end{tabular}
\caption{\textbf{Invalid instruments:} MAE, median bias, coverage, and mean LPS on 100 simulated datasets with $s$ invalid instruments. The best values in each column are printed in bold. The sisVIVE estimator does not provide any uncertainty quantification, so we do not report any coverage results.}
\label{tab:Kang_Sim}
\end{table}
